SIDEs: Separating Idealization from Deceptive Explanations in xAI

Explainable AI (xAI) methods are important for establishing trust in using black-box models. However, recent criticism has mounted against current xAI methods that they disagree, are necessarily false, and can be manipulated, which has started to undermine the deployment of black-box models. Rudin (2019) goes so far as to say that we should stop using black-box models altogether in high-stakes cases because xAI explanations "must be wrong". However, strict fidelity to the truth is historically not a desideratum in science. Idealizations -- the intentional distortions introduced to scientific theories and models -- are commonplace in the natural sciences and are seen as a successful scientific tool. Thus, it is not falsehood qua falsehood that is the issue. In this paper, I outline the need for xAI research to engage in idealization evaluation. Drawing on the use of idealizations in the natural sciences and philosophy of science, I introduce a novel framework for evaluating whether xAI methods engage in successful idealizations or deceptive explanations (SIDEs). SIDEs evaluates whether the limitations of xAI methods, and the distortions that they introduce, can be part of a successful idealization or are indeed deceptive distortions as critics suggest. I discuss the role that existing research can play in idealization evaluation and where innovation is necessary. Through a qualitative analysis we find that leading feature importance methods and counterfactual explanations are subject to idealization failure and suggest remedies for ameliorating idealization failure.

==> tabels/Phase_questions.tex <==
\begin{table}[ht]
\small
\centering
\caption{Relevant questions for each phase in SIDEs}
\label{table:phase_q}
% \begin{adjustbox}{angle=0}
\begin{tabular}{p{2cm}p{12cm} }
\toprule
\bf{SIDEs Phase}  & \bf{Evaluative questions} \\
\midrule

\textsc{Purpose} & \begin{itemize}
    \item What purpose does an xAI explanation have in this context?
    \item What purpose should an xAI explanation have in this context? 
    \item Example: Is an actionable explanation more suitable than an explanation that allows for contestability?
\end{itemize}
\\\\ 
\textsc{Idealization Practice} & What idealization practice is implicit in an given xAI method? What idealization practices are justified in a given context? 
\\\\
\textsc{Ideals} & What are the ideals and norms that govern a particular idealization practice? What are the different trade offs between different ways of operationalizing these ideals? 
\\\\
\textsc{Rules} & 
\\\\
\textsc{User-facing}
\textsc{explanations} & 
\\ 
\bottomrule
\end{tabular}
% \end{adjustbox}
\end{table}

==> tabels/Recourse.tex <==
\begin{table}[CE]
\small
\centering
\caption{Features of Idealization}
\label{table:CE}
% \begin{adjustbox}{angle=0}
\begin{tabular}{}
\toprule
\bf{\textsc{Purpose}}  & \bf{Misalignment} & \bf{\textsc{rule} failure} & \bf{explanation failure}\\
\midrule

\textsc{Epistemic} & x and y & C-ext  
\\\\
\textsc{Recourse} & \textsc{purpose-user-facing} 
\\ 
\bottomrule
\end{tabular}
% \end{adjustbox}
\end{table}

==> tabels/gi.tex <==
\begin{table}[gi]
\small
\centering
\caption{Features of Galilean Idealization}
\label{table:gi}
% \begin{adjustbox}{angle=0}
\begin{tabular}{  p{2.1cm}p{6cm} }
\toprule
\bf{Idealization 
\newline
Features}  & \bf{Galilean Idealization} \\
\midrule

Purpose & Pragmatic: simplifying to make problems more tractable
\\\\
Method & Simplify aspects of phenomena that later can be replaced with more accurate representations
\\\\
Justification & Make progress on a problem given pragmatic constraints, knowing that in the future when these constraints ease up a more accurate representation will follow 
\\\\
Ideals & Completeness    
\\\\
Rules & {\color{blue} The degree of precision and accuracy for judging models}
\\\\
Transient & Yes; idealizations must have a path to be de-idealized
\\\\ 
\bottomrule
\end{tabular}
% \end{adjustbox}
\end{table}

==> tabels/xai_eval.tex <==

\pagestyle{empty}
\renewcommand{\printlandscape}{\special{landscape}}
% \slideframe{none}
% \centerslidesfalse
% \slidesmag{3}
% \setlength{\slideheight}{183mm}
% \setlength{\slidewidth}{264mm}

\makeatletter
\newcommand{\armultirow}[3]{%
  \multicolumn{#1}{#2}{%
    \begin{picture}(0,0)%
      \put(0,0){%
        \begin{tabular}[t]{@{}#2@{}}%
          #3%
        \end{tabular}%
      }%
    \end{picture}%
  }%
}%

\newcolumntype{f}{>{$}l<{$}}
\newcolumntype{n}{l}
\newcolumntype{N}{>{\scriptsize}l}
\newcolumntype{v}[1]{>{\raggedright\hspace{0pt}}p{#1}}
\newcolumntype{V}[1]{>{\scriptsize\raggedright\hspace{0pt}}p{#1}}
%
% array.sty, dcolumn.sty
\newcolumntype{B}[1]{>{\boldmath\DC@{.}{,}{#1}}l<{\DC@end}}
\newcolumntype{d}[1]{>{\DC@{.}{,}{#1}}l<{\DC@end}}
\newcolumntype{i}[1]{>{\DC@{.}{,}{#1}\mathnormal\bgroup}l<{\egroup\DC@end}}
\newcolumntype{s}[1]{>{\DC@{.}{,}{#1}\mathsf\bgroup}l<{\egroup\DC@end}}
%
% array.sty, rotating.sty
\newcolumntype{R}[1]{%
  >{\begin{turn}{90}\begin{minipage}{#1}\scriptsize\raggedright\hspace{0pt}}l%
  <{\end{minipage}\end{turn}}%
}
%
% array.sty, tabularx.sty
\newcolumntype{x}{>{\scriptsize\raggedright\hspace{0pt}}X}
\makeatother
% \begin{document}

\begin{slide*}
  \begin{table}
    \centering
    \caption{Evaluating xAI with SIDEs}
    \label{tabel:xai_eval}
    \begin{tabular}{@{}v{7em}i{4.0}i{3.0}i{5.0}n@{}}
      \toprule
        % &
        \\
    %   \cmidrule(l){2-5}
        &
        \multicolumn{1}{V{5.5em}}{\textsc{purpose}} &
        \multicolumn{1}{V{5.5em}}{Misalignment} &
        \multicolumn{1}{V{5em}}{\textsc{Rule} failure} &
        \multicolumn{1}{V{5em}}{Success} 
        % &
        % &
        \multicolumn{1}{N}{\unit{}} \\
      \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}%
        \cmidrule(l){5-5}
        \armultirow{1}{@{}v{7em}}{LIME} &
          1991 & 20 & 45637 & \oldstylenums{657} unter  \\
        & 1992 & 47 & 47916 & \oldstylenums{645} linken \\
        & 1993 & 65 & 22848 & \oldstylenums{347} nein   \\
      \addlinespace
        \armultirow{1}{@{}v{7em}}{SHAP} &
          1994 &  87 & 46475 & \oldstylenums{957} einem  \\
        & 1995 &  95 & 94356 & \oldstylenums{8363} Sache \\
        & 1996 & 100 & 84646 & \oldstylenums{93635} nein \\
    \addlinespace
        \armultirow{1}{@{}v{7em}}{SHAP} &
          1994 &  87 & 46475 & \oldstylenums{957} einem  \\
        & 1995 &  95 & 94356 & \oldstylenums{8363} Sache \\
        & 1996 & 100 & 84646 & \oldstylenums{93635} nein \\
    \addlinespace
        \armultirow{1}{@{}v{7em}}{SHAP} &
          1994 &  87 & 46475 & \oldstylenums{957} einem  \\
        & 1995 &  95 & 94356 & \oldstylenums{8363} Sache \\
        & 1996 & 100 & 84646 & \oldstylenums{93635} nein \\
    %   \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}%
    %     \cmidrule(l){5-5}
    %     &
    %     \multicolumn{4}{N@{}}{Gerade langt hinauf sonst nicht gleich
    %       man} \\
    %   \cmidrule(r){1-1}\cmidrule(l){2-5}
    %     \armultirow{1}{@{}v{7em}}{Um hier damit Platz hat} &
    %       1796 &   4 & 46032 & \oldstylenums{56} scheidet \\
    %     & 1896 &  25 & 38937 & \oldstylenums{746} linken  \\
    %     & 1996 & 100 & 83458 & \oldstylenums{48746} eine  \\
      \bottomrule
    \end{tabular}
  \end{table}
\end{slide*}

